A model structure for locally constant factorization algebras

Several model structures related to the homotopy theory of locally constant factorization algebras are constructed. This answers a question raised by D. Calaque in his habilitation thesis. Our methods also solve a problem related to cosheafification and factorization algebras identified by O. Gwilliam - K. Rejzner in the locally constant case.

==> Contents/ComparisonLanForPMonoidalCats.tex <==
 This appendix is devoted to the comparison of derived left Kan extension and derived operadic left Kan extension along a symmetric monoidal functor between operads associated to a partial monoidal structure. We mainly follow \cite[Sections 1.2 and 2.2]{ayala_factorization_2017} with simple adaptations coming from the introduction of partial monoidal $\infty$-categories. The main result, Proposition \ref{prop_DerivedLanIsDerivedOperadicLanForPMonoidalCats}, will be essential for the construction of the factorization model in Section \ref{sect_WeissFactorizationModels}.
 
 In \cite{lurie_higher_2017}, Lurie proposed a fibrational description of symmetric monoidal $\infty$-categories.
 The idea is as follows: a (small) symmetric monoidal category $\Crect$ is a symmetric monoid in $\mathsf{Cat}$. This data can be encoded by a functor $\mathcal{F}_{\Crect}\colon \Fin_{*}\to\mathsf{Cat}$ satisfying Segal conditions, where $\Fin_{*}$ is the category of pointed finite sets. More explicitly, on objects $\mathcal{F}_{\Crect}\colon \langle\upn\rangle\mapsto \mathsf{C}^{\times \upn}$, and on arrows, $\mathcal{F}_{\Crect}$ sends:
 \begin{itemize}
 	\item surjective active maps to tensor products, e.g. $\boxtimes\colon\Crect^{\times\upn}\to \Crect$.
 	\item injective active maps to insertions of units, e.g. $\mathbb{I}_{\Crect}\colon\mathbb{1}\to \Crect$.
 	\item inert maps to projections of factors, e.g. $\textup{proj}_i\colon \Crect^{\times\upn}\to \Crect$.
 \end{itemize}
 Prescribing functoriality on those classes suffices, since every map in $\Fin_*$ factors (uniquely) as a surjective active map followed by an injective active map and finally an inert map. Moreover, Segal conditions on $\mathcal{F}_{\Crect}$ just ask that 
 $$
 \mathcal{F}_{\Crect}(\langle\upn\rangle)=\Crect^{\times\upn}\overset{\simeq}{\longrightarrow}\bigsqcap_{1\leq i\leq\upn}\Crect=\bigsqcap_{1\leq i\leq\upn}\mathcal{F}_{\Crect}(\langle 1 \rangle)
 $$
 via the family of inert maps $\uprho^i\colon\langle\upn\rangle\to\langle 1\rangle$ representing $i^{\textup{th}}$-factor projections. Via unstraightening, or Grothendieck construction, $\mathcal{F}_{\Crect}$ is presented alternatively as a cocartesian fibration  $\Crect^{\otimes}\to\Fin_{*}$ (satisfying Segal conditions). This way, cocartesian lifts of active/inert maps in $\Fin_{*}$ represent the structure described above for the functor $\mathcal{F}_{\Crect}$. Consult \cite{groth_short_2015} for more details.
 
 Hence, following Lurie:
 \begin{defn}\cite[Definition 2.0.0.7]{lurie_higher_2017}
 A \emph{symmetric monoidal $\infty$-category} is a cocartesian fibration of simplicial sets $\C^{\otimes}\to\Fin_*$ such that choosing cocartesian lifts for $(\uprho^i\colon \langle\upn\rangle\to\langle 1\rangle\text{ inert})_{1\leq i\leq \upn}$ yields an equivalence of $\infty$-categories
\begin{equation}\tag{Segal condition}
 (\uprho^i_!)_i\colon\C^{\otimes}_{\langle\upn\rangle}\overset{\sim}{\longrightarrow}\bigsqcap_{1\leq i\leq\upn}\C^{\otimes}_{\langle 1\rangle}=\bigsqcap_{1\leq i\leq\upn}\C.
\end{equation}
 \end{defn}

In a similar manner, $\infty$-operads are described by a fibrational structure.

\begin{defn}\cite[Definition 2.1.1.10]{lurie_higher_2017} 
An \emph{$\infty$-operad} is a map of simplicial sets $\Op^{\otimes}\to\Fin_{*}$ satisfying:
\begin{itemize}
	\item Restricted to the subcategory of inert maps, $\Op^{\otimes}_{\vert\mathsf{Inert}_*}\to \mathsf{Inert}_*$, it is a cocartesian fibration. Equivalently, there are cocartesian lifts for inert maps.
	\item Choosing cocartesian lifts for $(\uprho^i\colon \langle\upn\rangle\to\langle 1\rangle\text{ inert})_{1\leq i\leq \upn}$ yields an equivalence of $\infty$-categories
\begin{equation}\tag{Segal condition}
	(\uprho^i_!)_i\colon\Op^{\otimes}_{\langle\upn\rangle}\overset{\sim}{\longrightarrow}\bigsqcap_{1\leq i\leq\upn}\Op^{\otimes}_{\langle 1\rangle}=\bigsqcap_{1\leq i\leq\upn}\Op. 
\end{equation}
	\item For any pair of objects $\left[\upo_1,\dots,\upo_{\upn}\right]$,  $\left[\upu_1,\dots,\upu_{\upm}\right]\in\Op^{\otimes}$, the canonical map 
	%For any pair of objects $\underline{\upo}\simeq\left[\upo_1,\dots,\upo_{\upn}\right]$,  $\underline{\upu}\simeq\left[\upu_1,\dots,\upu_{\upm}\right]\in\Op^{\otimes}$, the canonical map of spaces 
%	$$
%	\Op^{\otimes}\brbinom{\underline{\upo}}{\underline{\upu}}\longrightarrow \bigsqcup_{\upf\in\Fin_{*}(\langle\upn\rangle,\langle\upm\rangle)}\bigsqcap_{1\leq j\leq\upm}\Op^{\otimes}\brbinom{\left[\upo_i\right]_{i\in\upf^{-1}(j)}}{\upu_j}
%	$$
	$$
	\Op^{\otimes}\brbinom{\left[\upo_1,\dots,\upo_{\upn}\right]}{\left[\upu_1,\dots,\upu_{\upm}\right]}\longrightarrow \bigsqcup_{\upf\in\Fin_{*}(\langle\upn\rangle,\langle\upm\rangle)}\bigsqcap_{1\leq j\leq\upm}\Op^{\otimes}\brbinom{\left[\upo_i\right]_{i\in\upf^{-1}(j)}}{\upu_j}
	$$
	is an equivalence of spaces.
\end{itemize}
\end{defn}
 
\begin{rem}
The main difference between both notions lies on the absence of operations parametrized by active maps in $\Fin_*$. As commented above, these correspond to tensor products, units and coherence data providing the axioms that define a symmetric monoidal structure.
\end{rem} 
 
Therefore, one can define partial (symmetric) monoidal $\infty$-categories as a hybrid where we choose what structure is required:
\begin{defn}
A \emph{partial monoidal $\infty$-category} is a replete $\infty$-subcategory inclusion over $\Fin_{*}$
$$
\begin{tikzcd}[ampersand replacement=\&]
\EuScript{S}_{\OpP}\ar[rr, hookrightarrow, "\textup{inc}"]\ar[rd, "\uppi_{\vert}"'] \&\& \OpP^{\otimes}\ar[ld,"\uppi"]\\
\& \Fin_*
\end{tikzcd}
$$
such that:
\begin{itemize}
	\item $\uppi\colon \OpP^{\otimes}\to \Fin_*$ is an $\infty$-operad.
	\item $\uppi_{\vert}\colon \EuScript{S}_{\OpP}\to \Fin_*$ is a cocartesian fibration.
	\item The inclusion $\EuScript{S}_{\OpP}\hookrightarrow\OpP^{\otimes}$ respects inert cocartesian maps and induces an equivalence between fibers over $\langle 0\rangle$ and $\langle 1\rangle$.
	\item Multimapping spaces $\OpP^{\otimes}\brbinom{\underline{\textup{a}}}{\textup{b}}$ are empty whenever $\underline{\textup{a}}$ does not belong to $\EuScript{S}_{\OpP}$.
%	
%	EQUIVALENTLY, for any object $\underline{a}\in \OpP^{\otimes}$ not in $\EuScript{S}$, its undercategory is initial, i.e. $\OpP^{\otimes}_{\underline{a}\slash}\simeq \mathbb{0}$.
\end{itemize}
% map of simplicial sets $\uppi\colon\OpP^{\otimes}\to\Fin_{*}$ with choices of full subcategories   $(\textup{S}_{\upn}\subseteq\OpP^{\otimes}_{\langle\upn\rangle})_{\upn}$ such that:
%\begin{itemize}
%	\item $\OpP^{\otimes}\to \Fin_*$ is an $\infty$-operad.
%	\item There are $\uppi$-cocartesian lifts for active maps with domain in $\textup{S}_{\upn}$ .
%	\item For any pair of objects $\underline{\upp}\in\OpP^{\otimes}_{\langle\upn\rangle}$,  $\upq\in\OpP^{\otimes}_{\langle 1\rangle}$, the mapping space 
%	$$
%	\OpP^{\otimes}\brbinom{\underline{\upp}}{\upq}=\left\lbrace
%	\begin{matrix}
%	\OpP^{\otimes}\brbinom{\underline{\upp}}{\upq} & \text{if }\underline{\upp} \text{ belongs to  }\textup{S}_{\upn},\\
%	\mathbb{0} & \text{otherwise.}
%	\end{matrix}
%	\right.
%	$$ 
%\end{itemize}
\end{defn}  

We explain this definition by means of a (discrete) fundamental  example.

\begin{ex} Let $\X$ be a topological space and $\Op(\X)$ its poset of open subsets seen as a category. Disjoint union of open sets determines a partial monoidal structure on $\Op(\X)$ since it is not defined for every pair of objects. Indeed, there is a partially defined functor (i.e. with domain in a subcategory) 
	$$
	\begin{tikzcd}[ampersand replacement=\&]
	\sqcup\colon \Op(\X)^{\times 2}\ar[r,dashed]\&\Op(\X),
	\end{tikzcd}
	$$
a unit $\o\in\Op(\X)$ and identities showing that it satisfies unitality and associativity when operations are defined. 

By analogy with symmetric monoidal categories, this structure can be encoded by two intertwining diagrams of categories:	$\mathcal{F}_{\Op(\X)}\colon \Fin_*^{\text{inert}}\to \mathsf{Cat}$ which codifies the family of categories $(\Op(\X)^{\times \upn})_{\upn}$ along with projections between them; and $\mathcal{F}_{\Op(\X)^{\text{djt}}}\colon\Fin_*\to\mathsf{Cat}$ codifying domains for the partial multiplications,  unit and identities for unitality and associativity. More concretely, $\mathcal{F}_{\Op(\X)}(\langle \upn\rangle)=\Op(\X)^{\times\upn}$ is the category of $\upn$-tuples of open subsets in $\X$ and $\mathcal{F}_{\Op(\X)^{\text{djt}}}(\langle\upn\rangle)$ its full subcategory spanned by pairwise disjoint $\upn$-tuples of open subsets. Functoriality of $\mathcal{F}_{\Op(\X)^{\text{djt}}}$ over active maps determine the partial monoidal structure.

The Grothendieck construction associates to $\mathcal{F}_{\Op(\X)^{\text{djt}}}$ a cocartesian fibration $\Op(\X)^{\text{djt}}\to \Fin_{*}$, whereas the functor $\Op(\X)^{\otimes}\to\Fin_*$ is the category of operators associated to $\Op(\X)$ with its inherited operad structure. Being more explicit, the operadic structure is just
$$
\Op(\X)\brbinom{\{\mathsf{U}_i\}_i}{\mathsf{V}}=\left\{\begin{matrix}
\mathbb{1} & \;\text{ if }\bigsqcup_i\mathsf{U}_i\subseteq \mathsf{V}\\\\
\mathbb{0} & \;\text{ else,}
\end{matrix}\right.
$$
with obvious composition laws, and the category of operators satisfies
$$
\Op(\X)^{\otimes}\brbinom{\left[\mathsf{U}_1,\dots,\mathsf{U}_{\upn}\right]}{\left[\mathsf{V}_1,\dots,\mathsf{V}_{\upm}\right]}\overset{\simeq}{\longrightarrow} \bigsqcup_{\upf\in\Fin_{*}(\langle\upn\rangle,\langle\upm\rangle)}\bigsqcap_{1\leq j\leq\upm}\Op(\X)\brbinom{\left\lbrace\mathsf{U}_i\right\rbrace_{i\in\upf^{-1}(j)}}{\mathsf{V}_j}.
$$	

It is clear that we obtain a replete subcategory inclusion over $\Fin_*$,
$$
\begin{tikzcd}[ampersand replacement=\&]
\Op(\X)^{\text{djt}}\ar[rr, hookrightarrow]\ar[rd, ""'] \&\& \Op(\X)^{\otimes}\ar[ld,""]\\
\& \Fin_*
\end{tikzcd}
$$

The first three axioms in the above definition are immediate. The fourth just forces $\Op(\X)^{\otimes}$ to have no more operations than the ones which come from the partial monoidal structure. 
\end{ex}

Note that symmetric monoidal $\infty$-categories are also  examples of partial monoidal $\infty$-categories, and as them, they admit two notions of morphism between them.

\begin{defn} A morphism 
	$\EuScript{S}_{\mathfrak{B}}\subseteq\mathfrak{B}^{\otimes}\to \mathfrak{N}^{\otimes}\supseteq\EuScript{S}_{\mathfrak{N}}$ over $\Fin_{*}$ between partial monoidal $\infty$-categories is a:
	\begin{itemize}
		\item \emph{lax monoidal functor} if it sends inert cocartesian arrows to cocartesian arrows and restricts to a map $\EuScript{S}_{\mathfrak{B}}\to\EuScript{S}_{\mathfrak{N}}$.
		\item \emph{strong monoidal functor} if it is lax monoidal and the restriction $\EuScript{S}_{\mathfrak{B}}\to\EuScript{S}_{\mathfrak{N}}$ preserves cocartesian arrows over $\Fin_*$.
	\end{itemize}
\end{defn}
 
We introduce partial monoidal structures in order to obtain a slight generalization of \cite[Lemma 2.16]{ayala_factorization_2017}.
 \begin{lem}\label{lem_AyalaFrancisTanakaLemmaForPMonoidalInftyCategories}
 Let $\mathfrak{V}$ be a cocomplete symmetric monoidal $\infty$-category such that its tensor product distributes colimits on both variables and let $\upiota\colon \mathfrak{B}\to\mathfrak{N}$ be a strong monoidal functor between partial monoidal $\infty$-categories. Then, the horizontal functors in the commutative solid square below admit left adjoints 
 $$
 \begin{tikzcd}[ampersand replacement=\&]
 \Fun(\mathfrak{B},\mathfrak{V})\ar[rr, bend left=10, " \upiota_!", dashed]\&\& \Fun(\mathfrak{N},\mathfrak{V})\ar[ll, bend left=10]\\ \\
 \Fun^{\textup{lax}}(\mathfrak{B},\mathfrak{V})\ar[rr, bend left=10, " \upiota_{\sharp}", dashed]\ar[uu, "\textup{forget}"]\& \& \,\Fun^{\textup{lax}}(\mathfrak{N},\mathfrak{V}).\ar[uu, "\textup{forget}"']\ar[ll, bend left=10]
 \end{tikzcd}
 $$
 Moreover, the square of decorated arrows also commutes, the upper left adjoint is
 $$
 \upiota_!\F\,(\Z)\simeq \underset{\mathfrak{B}_{\downarrow\Z}}{\hocolim}\,\F(\upb)
 $$
 and $\upiota_!$, $\upiota_\sharp$ are fully-faithful if $\upiota$ is so.
 
 The same conclusions hold replacing lax monoidal functors by strong monoidal functors provided:
 \begin{itemize}
 \item for any $\left[\Z_1,\dots,\Z_{\upn}\right]\in\EuScript{S}_{\langle\upn\rangle}$, the canonical functor
 $$
\mathfrak{B}_{\downarrow\Z_1}\times\cdots\times\mathfrak{B}_{\downarrow\Z_{\upn}}\longrightarrow\mathfrak{B}_{\downarrow(\Z_1\boxtimes\cdots\boxtimes\,\Z_{\upn})} 
 $$
 is final, and 
 \item	the object 
 $
(\mathbb{I}_{\mathfrak{B}}, \upiota(\mathbb{I}_{\mathfrak{B}})\xrightarrow{\upiota\textup{-strong}}\mathbb{I}_{\mathfrak{N}})\in \mathfrak{B}_{\downarrow\mathbb{I}_{\mathfrak{N}}}
 $ 
 is terminal.
 \end{itemize}
 \end{lem}
\begin{proof} The proof is an adaptation of \cite[Lemma 2.16]{ayala_factorization_2017}.
	
 First, $\upiota_!$ exists since such pointwise formula provides the left adjoint by cocompleteness of $\mathfrak{V}$ (see \cite[Lemma 4.3.2.13]{lurie_higher_2009}). 
	
 Next, we must show that $\upiota_!$ restricts to lax monoidal functors. That is, it suffices to check that for $\F$ lax monoidal, $\upiota_!\F$ is lax monoidal as well. %; that is to say: $\upiota_!\F$ preserves inert cocartesian arrows.
  Diagramatically, this means that the squares
   $$
  \begin{tikzcd}[ampersand replacement=\&]
 \mathfrak{N}_{\langle \upn\rangle}^{\otimes} \ar[rr,"(\upiota_!\F)_{\langle\upn\rangle}"]\ar[d,"\upf_!"']\&\& \mathfrak{V}^{\otimes}_{\langle\upn\rangle} \ar[d,"\upf_!"]\\
 \mathfrak{N}_{\langle \upt\rangle}^{\otimes} \ar[rr,"(\upiota_!\F)_{\langle\upt\rangle}"']\&\& \mathfrak{V}^{\otimes}_{\langle\upt\rangle} 
  \end{tikzcd}
  $$ 
% $$
% \begin{tikzcd}[ampersand replacement=\&]
%\bigsqcap_{i}\mathfrak{N} \& \mathfrak{N}_{\langle \upn\rangle}^{\otimes} \ar[rr,"(\upiota_!\F)_{\langle\upn\rangle}"]\ar[l,"\sim"']\ar[d,"\upf_!"']\&\& \mathfrak{V}^{\otimes}_{\langle\upn\rangle} \ar[r,"\sim"]\ar[d,"\upf_!"]\& \bigsqcap_i
%\mathfrak{V}\\
%\bigsqcap_{j}\mathfrak{N} \& \mathfrak{N}_{\langle \upt\rangle}^{\otimes} \ar[rr,"(\upiota_!\F)_{\langle\upt\rangle}"']\ar[l,"\sim"]\&\& \mathfrak{V}^{\otimes}_{\langle\upt\rangle} \ar[r,"\sim"']\& \bigsqcap_j
%\mathfrak{V}
% \end{tikzcd}
% $$ 
 are commutative, where $\upf\colon \langle\upn\rangle\to\langle\upt\rangle$ is inert in $\Fin_*$ and the vertical arrows are induced by choosing cocartesian lifts over $\upf$. By Segal conditions, $\mathfrak{N}^{\otimes}_{\langle\upn\rangle}\simeq \bigsqcap_i\mathfrak{N}$ respectively  $\mathfrak{V}^{\otimes}_{\langle\upn\rangle}\simeq \bigsqcap_i\mathfrak{V}$, the vertical maps are just projections onto some factors and thus the claim is obvious.  
 
 Let us explore what is the lax monoidal structure that $\upiota_!\F$ inherits in more concrete terms. For $\upg\colon \colon \langle\upn\rangle\to\langle\upm\rangle$ active, choosing cocartesian lifts also produces a rectangle of $\infty$-categories
  $$
\begin{tikzcd}[ampersand replacement=\&]
(\EuScript{S}_{\mathfrak{N}})_{\langle\upn\rangle}\ar[r,hookrightarrow]\ar[d,"\upg_!"'] \& \mathfrak{N}_{\langle \upn\rangle}^{\otimes} \ar[rr,"(\upiota_!\F)_{\langle\upn\rangle}"]\&\& \mathfrak{V}^{\otimes}_{\langle\upn\rangle} \ar[d,"\upg_!"]\\
(\EuScript{S}_{\mathfrak{N}})_{\langle\upm\rangle}\ar[r,hookrightarrow] \& \mathfrak{N}_{\langle \upm\rangle}^{\otimes} \ar[rr,"(\upiota_!\F)_{\langle\upm\rangle}"']\&\& \,\mathfrak{V}^{\otimes}_{\langle\upm\rangle},
\end{tikzcd}
  $$ 
 but it need not be commutative. However, the universal property of cocartesian lifts gives rise to a natural transformation $\upg_!\cdot(\upiota_!\F)_{\langle\upn\rangle} \cdot\textup{inc}\Rightarrow (\upiota_!\F)_{\langle\upm\rangle}\cdot\textup{inc}\cdot\upg_!$ filling the above rectangle. Let us see what are the  components of this natural transformation for some active maps.  
 
\begin{itemize} 
\item For the unique $\upg\colon\langle 0\rangle\to \langle 1\rangle $, the component of the transformation is given by the unit map for $\upiota_!\F$:
$$
\mathbb{I}_{\mathfrak{V}}\xrightarrow{\F\textup{-lax monoidal}}\mathsf{F}(\mathbb{I}_{\mathfrak{B}})\xrightarrow{\textup{adjunction}}\upiota_!\F(\upiota(\mathbb{I}_{\mathfrak{B}}))\xrightarrow{\upiota\textup{-strong monoidal}}\upiota_!\F(\mathbb{I}_{\mathfrak{N}}).
$$
\item For the active map $\upg\colon\langle \upn\rangle\to \langle 1\rangle$ sending everything different from the basepoint to 1, the component of the natural transformation at an object $\left[\Z_1,\dots,\Z_{\upn}\right]\in\EuScript{S}_{\langle\upn\rangle}$, it is given by the multiplication map

\begin{tikzcd}[ampersand replacement=\&]
\upiota_!\F(\Z_1)\otimes\cdots\otimes\upiota_!\F(\Z_{\upn})\ar[r,equal]\&\underset{\mathfrak{B}_{\downarrow\Z_1}}{\hocolim}\,\F(\upb_1)\otimes\cdots\otimes\underset{\mathfrak{B}_{\downarrow\Z_{\upn}}}{\hocolim}\,\F(\upb_{\upn})\ar[d,"\otimes\textup{-cocontinuous}","\simeq"']\\
	\&\underset{\mathfrak{B}_{\downarrow\Z_1}\times\cdots\times\mathfrak{B}_{\downarrow\Z_{\upn}}}{\hocolim}\,\F(\upb_1)\otimes\cdots\otimes\,\F(\upb_{\upn})\ar[d,"\F\textup{-lax monoidal}"]\\
	\&\underset{\mathfrak{B}_{\downarrow\Z_1}\times\cdots\times\mathfrak{B}_{\downarrow\Z_{\upn}}}{\hocolim}\,\F(\upb_1\boxtimes\cdots\boxtimes\upb_{\upn})\ar[d,"\upiota\textup{-strong monoidal}", "\textup{partial monadicity}"']\\
\upiota_!\F(\Z_1\boxtimes\cdots\boxtimes\Z_{\upn})\ar[r,equal]	\&\underset{\mathfrak{B}_{\downarrow(\Z_1\boxtimes\cdots\boxtimes\,\Z_{\upn})}}{\hocolim}\,\F(\upb).
	\end{tikzcd}
\end{itemize}

Thus, this is just the lax monoidal structure of $\upiota_!\F$. The coherence is encoded on the interaction of all active maps in $\Fin_*$, which can be seen as combinations of the above mentioned simple cases. 

For the strong monoidal case, $\upiota_!\F$ must be strong monoidal when $\F$ is so. Hence, by the above analysis, we are reduced to prove that the natural transformation just described is a natural equivalence. It suffices to see that its components are equivalences. The explicit given description together with the assumptions on the statement conclude the lemma.

\end{proof}

 
\begin{prop}\label{prop_DerivedLanIsDerivedOperadicLanForPMonoidalCats}
Let $\V$ be a homotopy cosmos where $\Upsigma$-cofibrant operads are admissible (Hypothesis \ref{hyp_VNiceEnough}). Let $\upiota\colon \OpB\to\OpN$ be a strong monoidal functor between partial monoidal $\sSet$-categories with underlying $\Upsigma$-cofibrant operads. Then, the following square of decorated functors is commutative (up to equivalence)
		$$
		\begin{tikzcd}[ampersand replacement=\&]
		\Alg_{\overline{\OpB}}(\V)\ar[rr, bend left=10, " \mathbb{L}\upiota_!"]\&\& \Alg_{\overline{\OpN}}(\V)\ar[ll, bend left=10]\\ \\
		\Alg_{\OpB}(\V)\ar[rr, bend left=10, " \mathbb{L}\upiota_{\sharp}"]\ar[uu, "\overline{\star}"]\& \& \,\Alg_{\OpN}(\V).\ar[uu, "\overline{\star}"']\ar[ll, bend left=10]
		\end{tikzcd}
		$$
		In other words, there is a natural equivalence 
		$
		\mathbb{L}\upiota_!\overline{\Aalg}\simeq \overline{\mathbb{L}\upiota_{\sharp}\Aalg}.
		$
 \end{prop}
 \begin{proof}
 	The admissibility hypothesis says that the square of model categories and right Quillen functors
 	$$
 	\begin{tikzcd}[ampersand replacement=\&]
 	\Alg_{\overline{\OpB}}(\V)_{\textup{proj}}\&\& \Alg_{\overline{\OpN}}(\V)_{\textup{proj}}\ar[ll, bend left=10,"\upiota^*"]\\ \\
 	\Alg_{\OpB}(\V)_{\textup{proj}}\ar[uu, "\overline{\star}"]\& \& \,\Alg_{\OpN}(\V)_{\textup{proj}}.\ar[uu, "\overline{\star}"']\ar[ll, bend left=10,"\upiota^*"]
 	\end{tikzcd}
 	$$
    exists. We should check that it	represents the solid square in Lemma \ref{lem_AyalaFrancisTanakaLemmaForPMonoidalInftyCategories} for its associated higher categorical version. This fact is a consequence of \cite[Theorem 4.10]{haugseng_algebras_2019}, since simplicial operads are colorwise cofibrant and cofibrant objects are flat in $\V$ for whatever choosen subcategory of flat objects. 
    
    By uniqueness of adjoints, the higher categorical version of both squares is essentially the same, up to a contractible space of choices.
    
    %The projective model on functor categories represents $\infty$-functors due to \cite[Proposition 4.2.4.4]{lurie_higher_2009}. The analogous result for operadic algebras is the content of \cite[Theorem 7.11]{pavlov_admissibility_2018}. By uniqueness of adjoints, the higher categorical version of both squares is essentially the same and hence, we may conclude.
 \end{proof}
 
 \begin{rem} In \cite[Proposition 4.2.4.4]{lurie_higher_2009} it is discussed when does the projective model on functor categories with a combinatorial codomain represent $\infty$-functors. The analogous result for operadic algebras is the content of \cite[Theorem 7.11]{pavlov_admissibility_2018}, obviously under several assumptions.
 	
 In this case, we preferred \cite[Theorem 4.10]{haugseng_algebras_2019} for its fewer requirements. 
 \end{rem}
 

 
 
 
 
 
 
 
 
% 
% Let $\upiota\colon \OpP\to\Op$ be a strong symmetric monoidal functor between partial symmetric monoidal categories. We want to compare (derived) ordinary Kan extension and (derived) operadic Kan extension along $\upiota$.
%
%We are going to exploit the following result.
%\begin{lem}\label{lem_AlgebrasOverPMonoidalCat}
%	The category of $\Op$-algebras is equivalent to that of $\overline{\Op}$-functors with (partial) lax monoidal structure. Symbollically,
%	$$
%	\Alg_{\Op}(\V)\simeq \left[\overline{\Op},\V\right]^{\mathsf{plax}}
%	$$
%\end{lem}
%\begin{proof} Unwrapping definitions of both categories, one finds that the claim reduces to the natural equivalence
%	$$
%	\Op\brbinom{\left[\upo_r\right]_r}{\upu}\cong \overline{\Op}\brbinom{\boxtimes_r\upo_r}{\upu} , 
%	$$
%	due to $\Op$ being (partial) symmetric monoidal category. In other words, nonunary operations are completely described by the universal operations $\id_{\underline{\upo}}\in\Op\brbinom{\left[\upo_r\right]_r}{\boxtimes_r\upo_r}$.
%\end{proof}	
%
%With this in mind, the non-homotopical result is easy.
%\begin{lem}\label{lem_LanIsOperadicLanForPMonoidalCats}
%	%  The Kan extension/restriction adjunction
%	%     	$
%	%     	\upiota_!\colon \Alg_{\overline{\OpP}}\rightleftarrows\Alg_{\overline{\Op}}\colon\upiota^*
%	%     	$
%	%     	restricts to an adjunction for operadic algebras
%	%        $
%	%     	\upiota_!\colon \Alg_{\OpP}\rightleftarrows\Alg_{\Op}\colon\upiota^*.
%	%     	$
%	%In other words, $\overline{\upiota_{\sharp}\Aalg}\cong \upiota_!\overline{\Aalg}$ for any $\mathsf{A}\in\Alg_{\OpP}$.
%	The following square of decorated functors is commutative
%	$$
%	\begin{tikzcd}[ampersand replacement=\&]
%	\Alg_{\overline{\OpP}}\ar[rr, bend left=10, " \upiota_!"]\&\& \Alg_{\overline{\Op}}\ar[ll, bend left=10]\\ \\
%	\Alg_{\OpP}\ar[rr, bend left=10, " \upiota_{\sharp}"]\ar[uu, "\overline{\star}"]\& \& \,\Alg_{\Op}.\ar[uu, "\overline{\star}"']\ar[ll, bend left=10]
%	\end{tikzcd}
%	$$
%	In other words, there is a natural isomorphism 
%	$
%	\upiota_!\overline{\Aalg}\simeq \overline{\upiota_{\sharp}\Aalg}.
%	$
%\end{lem}	
%%     	\begin{proof} We check that by factorizing $\upiota$ through its image $\OpI$, obtaining that each left adjoint decomposes as a composite
%%     		$$
%%     		\Alg_{\OpP}\underset{\textup{of colors}}{\xrightarrow{\textup{extension}}}\Alg_{\OpI}\underset{\textup{of operations}}{\xrightarrow{\textup{extension}}}\Alg_{\Op}.
%%     		$$
%%     		Since both extensions of colors, the one associated to $\upiota_!$ and the corresponding to $\upiota_{\sharp}$, yield a commutative square, it suffices to analyze extensions of operations. Let us employ $\circ$-product notation as in Section \ref{sect_FactHom}. Then, we should prove that the natural morphism 
%%     		$$
%%     		\overline{\Op}\underset{\overline{\OpI}}{\circ}\overline{\Aalg}\longrightarrow\overline{\Op\underset{\OpI}{\circ}\Aalg}
%%     		$$
%%     		is an iso for any $\OpI$-algebra $\Aalg$. Expanding the coequalizer description of relative $\circ$-product and the (unbiased) definition of $\circ$-product
%%     		$$
%%     			\begin{tikzcd}[ampersand replacement=\&]
%%     		\underset{\upu,\upo}{\bigsqcup}\,\,\overline{\Op}\brbinom{\upu}{\textup{v}}\otimes\overline{\OpI}\brbinom{\upo}{\upu}\otimes \Aalg(\upo)\ar[d,Rightarrow]\ar[rd,"\textup{factor inclusion}", bend left=5]\\  \underset{\upu}{\bigsqcup}\,\,\overline{\Op}\brbinom{\upu}{\textup{v}}\otimes \Aalg(\upu)\ar[d,"\text{coeq}"]\ar[rd, bend left=5] \& \underset{\brbinom{\underline{\upo}}{\underline{\upu}}}{\colim}\,\,\Op\brbinom{\underline{\upu}}{\textup{v}}\otimes\bigotimes_{j}\OpI\brbinom{\underline{\upo}_{\vert j}}{\upu_j}\otimes \bigotimes_{k_j}\Aalg(\upo_{k_j})\ar[d,Rightarrow]\\  \Big(\overline{\Op}\,\underset{\overline{\OpI}}{\circ}\,\overline{\Aalg}\Big)(\textup{v}) \ar[rd, dashed, bend left=5]\& \underset{\underline{\upu}}{\colim}\,\,\Op\brbinom{\underline{\upu}}{\textup{v}}\otimes\bigotimes_{j} \Aalg(\upu_j)\ar[d,"\text{coeq}"]\\
%%     		\& \,\Big(\overline{\Op\,\underset{\OpI}{\circ}\,\Aalg}\Big)(\textup{v}),
%%     		\end{tikzcd}
%%     		$$
%%     		we get that the natural morphism under inspection is the dashed arrow induced between coequalizers. There is a canonical retraction of the horizontal arrows given by the lax monoidal structure of $\Aalg$ plus (partial) symmetric monoidal structure of $\Op$ and $\OpI$ together with $\upiota$ being strong monoidal. For example, the above horizontal map is induced by
%%     		$$
%%     		\hspace*{-4mm}\overline{\Op}\brbinom{\boxtimes_j\upu_j}{\textup{v}}\otimes\,\overline{\OpI}\brbinom{\boxtimes_{k}\upo_{k}}{\boxtimes_j\upu_j}\otimes\, \Aalg(\boxtimes_{k}\upo_{k})\xleftarrow{\id\otimes \textup{tensor}_{\OpI}\otimes \textup{lax monoidal}} \Op\brbinom{\underline{\upu}}{\textup{v}}\otimes\,\bigotimes_{j}\OpI\brbinom{\underline{\upo}_{\vert j}}{\upu_j}\otimes\, \bigotimes_{k_j}\Aalg(\upo_{k_j}).
%%     		$$  
%%     		The compatibility with vertical arrows is immediate just as retraction condition.
%%     		
%%     		It remains to show that the composite
%%     		$$
%%     		\Big(\overline{\Op\,\underset{\OpI}{\circ}\,\Aalg}\Big)(\textup{v})\longrightarrow\Big(\overline{\Op}\,\underset{\overline{\OpI}}{\circ}\,\overline{\Aalg}\Big)(\textup{v})\longrightarrow\Big(\overline{\Op\,\underset{\OpI}{\circ}\,\Aalg}\Big)(\textup{v})
%%     		$$
%%     		equals the identity. Choosing a generalized element $\upt\colon \star\to\Big(\overline{\Op\,\underset{\OpI}{\circ}\,\Aalg}\Big)(\textup{v})$, we are reduced to see if the composite on $\upt$ equals $\upt$.
%%     		$$
%%     		\upt\mapsto (\textup{inclusion})\big(\id\otimes\,\textup{lax}\big)(\upt)
%%     		$$
%%     	\end{proof}
%\begin{proof}
%	By the universal property satisfied by $\upiota_{\sharp}\Aalg$, one could verify the claim by equipping $\upiota_!\overline{\Aalg}$ with a lax monoidal structure and showing that it is universal. The unit comes from the composite
%	$$
%	\mathbb{I}_{\V}\xrightarrow{\Aalg\textup{-lax}}\Aalg(\mathbb{I}_{\OpP})\xrightarrow{\textup{unit}}\upiota_!\overline{\Aalg}(\upiota(\mathbb{I}_{\OpP}))\xrightarrow{\upiota\textup{-colax}}\upiota_!\overline{\Aalg}(\mathbb{I}_{\Op})
%	$$
%	and the multiplication corresponds to the composite
%	$$
%	\begin{tikzcd}[ampersand replacement=\&]
%	\upiota_!\overline{\Aalg}(\upo_1)\otimes\upiota_!\overline{\Aalg}(\upo_2)\ar[d,equal]\\
%	\big(\int^{\upb_1}\Op\brbinom{\upiota\upb_1}{\upo_1}\otimes\Aalg(\upb_1)\big)\otimes\big(\int^{\upb_2}\Op\brbinom{\upiota\upb_2}{\upo_2}\otimes\Aalg(\upb_2)\big)\ar[d,"\textup{ Fubini, }\otimes\textup{-cocontinuous, symmetry}","\cong"']\\
%	\int^{\upb_1,\upb_2}\Op\brbinom{\upiota\upb_1}{\upo_1}\otimes\Op\brbinom{\upiota\upb_2}{\upo_2}\otimes \Aalg(\upb_1)\otimes\Aalg(\upb_2)\ar[d,"\textup{tensor}\,\otimes\,\textup{lax monoidal}"]\\
%	\int^{\upb_1,\upb_2}\Op\brbinom{\upiota\upb_1\boxtimes\,\upiota\upb_2}{\upo_1\boxtimes\upo_2}\otimes \Aalg(\upb_1\boxtimes\upb_2)\ar[d,"\textup{colax structure}\,\otimes\, \id"]\\
%	\int^{\upb_1,\upb_2}\Op\brbinom{\upiota(\upb_1\boxtimes\,\upb_2)}{\upo_1\boxtimes\upo_2}\otimes \Aalg(\upb_1\boxtimes\upb_2)\ar[d,"\cong"',"\textup{coYoneda lemma}"]\\
%	\int^{\upb_1,\upb_2}\Op\brbinom{\upiota(\upb_1\boxtimes\,\upb_2)}{\upo_1\boxtimes\upo_2}\otimes \Big(\int^{\upb}\OpP\brbinom{\upb}{\upb_1\boxtimes\,\upb_2}\otimes\Aalg(\upb)\Big)\ar[d,"\textup{ Fubini, }\otimes\textup{-cocontinuous}","\cong"']\\
%	\int^{\upb}\Big(\int^{\upb_1,\upb_2}\Op\brbinom{\upiota(\upb_1\boxtimes\,\upb_2)}{\upo_1\boxtimes\upo_2}\otimes \OpP\brbinom{\upb}{\upb_1\boxtimes\,\upb_2} \Big)\otimes \Aalg(\upb)\ar[d,"\textup{composition}\,\otimes\id"]\\
%	\int^{\upb}\Op\brbinom{\upiota\upb}{\upo_1\boxtimes\upo_2}\otimes \Aalg(\upb)\ar[d,equal]\\
%	\upiota_!\overline{\Aalg}(\upo_1\boxtimes\upo_2).
%	\end{tikzcd}
%	$$ 
%	Checking that these choices fulfil the requirements is a lenghty but straightforward computation.
%	%  $$
%	%  \begin{tikzcd}[ampersand replacement=\&]
%	%  \bigotimes_{r}\upiota_!\Aalg(\upo_r)\ar[d,"\textup{ Fubini, }\otimes\textup{-cocontinuous, symmetry}","\cong"']\\
%	%  \int^{(\upp_r)_r}\bigotimes_r\Op\brbinom{\upp_r}{\upo_r}\otimes \bigotimes_{r}\Aalg(\upp_r)\ar[d,"\textup{tensor}\,\otimes\,\textup{lax}"]\\
%	%  \int^{(\upp_r)_r}\Op\brbinom{\boxtimes_r\upp_r}{\boxtimes_r\upo_r}\otimes \Aalg(\boxtimes_r\upp_r)\ar[d,"\cong"',"\textup{coYoneda lemma}"]\\
%	%  \int^{(\upp_r)_r}\Op\brbinom{\boxtimes_r\upp_r}{\boxtimes_r\upo_r}\otimes \Big(\int^{\upp}\Op\brbinom{\upp}{\boxtimes_r\upp_r}\otimes\Aalg(\upp)\Big)\ar[d,"\textup{ Fubini, }\otimes\textup{-cocontinuous}","\cong"']\\
%	%  \int^{\upp}\Big(\int^{(\upp_r)_r}\Op\brbinom{\boxtimes_r\upp_r}{\boxtimes_r\upo_r}\otimes \Op\brbinom{\upp}{\boxtimes_r\upp_r} \Big)\otimes \Aalg(\upp)\ar[d,"\textup{composition}\,\otimes\id"]\\
%	%  \int^{\upp}\Op\brbinom{\upp}{\boxtimes_r\upo_r}\otimes \Aalg(\upp)\ar[d,equal]\\
%	%  \upiota_!\Aalg(\boxtimes_r\upo_r).
%	%  \end{tikzcd}
%	%  $$ 
%\end{proof}
%%     \begin{rem} This lemma is analogous to \cite[Lemma 2.16]{ayala_factorization_2017}. The advantages that it present is that it works for enrichments different from spaces and that it drops most of the assumptions that they consider. 
%%     \end{rem}	
%
%Our goal becomes verifying that the natural isomorphism $\upiota_!\overline{\Aalg}\cong\overline{\upiota_{\sharp}\Aalg} $ holds, possibly as an equivalence, when replacing left adjoints by their homotopical analogues. Equivalently, comparing derived Kan extensions. For this homotopical analysis, we will need some assumptions, see Remark at the end of section.
